Low Complexity Detection of Spatial Modulation Aided OTFS in Doubly-Selective Channels

A spatial modulation-aided orthogonal time frequency space (SM-OTFS) scheme is proposed for high-Doppler scenarios, which relies on a low-complexity distance-based detection algorithm. We first derive the delay-Doppler (DD) domain input-output relationship of our SM-OTFS system by exploiting an SM mapper, followed by characterizing the doubly-selective channels considered. Then we propose a distance-based ordering subspace check detector (DOSCD) exploiting the \emph{a priori} information of the transmit symbol vector. Moreover, we derive the discrete-input continuous-output memoryless channel (DCMC) capacity of the system. Finally, our simulation results demonstrate that the proposed SM-OTFS system outperforms the conventional single-input-multiple-output (SIMO)-OTFS system, and that the DOSCD conceived is capable of striking an attractive bit error ratio (BER) vs. complexity trade-off.

==> acronyms.tex <==
%
%acronyms

\newacronym{AWGN}{AWGN}{additive white Gaussian noise}

\newacronym{BABF}{BABF}{blind adaptive beamforming}

\newacronym{BER}{BER}{bit error ratio}

\newacronym{CW}{CW}{continuous wave}

\newacronym{CU}{CU}{control unit}

\newacronym{JML}{JML}{joint maximum-likelihood}

\newacronym{DPSK}{DPSK}{differential phase shift key}

\newacronym{PSK}{PSK}{phase shift key}

\newacronym{EM}{EM}{expectation maximization}

\newacronym{PDF}{PDF}{probability density function}

\newacronym{CSI}{CSI}{channel state information}

\newacronym{EPC}{EPC}{electronic product code}

\newacronym{RF}{RF}{radio frequency}

\newacronym{RIP}{RIP}{rotational invariance property}

\newacronym{RFID}{RFID}{radio frequency identification}

\newacronym{IC}{IC}{integrated circuit}

\newacronym{IoTs}{IoTs}{Internet of Things}

\newacronym{ULA}{ULA}{uniform linear array}

\newacronym{UHF}{UHF}{ultra high frequency}

\newacronym{OLS}{OLS}{ordinary least square}

\newacronym{QCQPs}{QCQPs}{quadratically constrained quadratic programs}

\newacronym{SDR}{SDR}{semidefinite relaxation}

\newacronym{SCA}{SCA}{successive convex approximation}

\newacronym{WET}{WET}{wireless energy transfer}

\newacronym{UWB}{UWB}{ultrawide bandwidth}

\newacronym{ToA}{ToA}{time-of-arrival}

\newacronym{PoA}{PoA}{phase-of-arrival}

\newacronym{DoA}{DoA}{direction-of-arrival}

\newacronym{RSS}{RSS}{received signal strength}

\newacronym{MSE}{MSE}{mean square error}

\newacronym{DoF}{DoF}{degree of freedom}

\newacronym{UAV}{UAV}{unmanned aerial vehicle}

\newacronym{CAMs}{CAMs}{cooperative awareness messages}

\newacronym{BS}{BS}{base station}

\newacronym{ID}{ID}{identification}

\newacronym{PL}{PL}{platoon leader}

\newacronym{PM}{PM}{platoon member}
\newacronym{PMs}{PMs}{platoon members}

\newacronym{a.k.a.}{a.k.a.}{also know as}

\newacronym{DPM}{DPM}{disconnected platoon member}

\newacronym{BaS}{BaS}{Braking and Stopping}

\newacronym{TAs}{TAs}{transmit antennas}

\newacronym{RAs}{RAs}{receive antennas}

\newacronym{3D}{3D}{three-dimensional}

\newacronym{ACK}{ACK}{acknowledgement}

\newacronym{V2V}{V2V}{vehicle-to-vehicle}

\newacronym{V2I}{V2I}{vehicle-to-infrastructure}

\newacronym{WLAN}{WLAN}{wireless local area network}

\newacronym{UAVs}{UAVs}{unmanned aerial vehicles}

\newacronym{ML}{ML}{machine learning}

\newacronym{TOA}{TOA}{time of arrival}

\newacronym{UWB}{UWB}{ultrawideband}

\newacronym{OBU}{OBU}{on-board unit}

\newacronym{LOS}{LOS}{line-of-sight}

\newacronym{RIB}{RIB}{rotational invariance beamforming}




















